Switching Head-Tail Funnel UNITER for Dual Referring Expression Comprehension with Fetch-and-Carry Tasks

This paper describes a domestic service robot (DSR) that fetches everyday objects and carries them to specified destinations according to free-form natural language instructions. Given an instruction such as "Move the bottle on the left side of the plate to the empty chair," the DSR is expected to identify the bottle and the chair from multiple candidates in the environment and carry the target object to the destination. Most of the existing multimodal language understanding methods are impractical in terms of computational complexity because they require inferences for all combinations of target object candidates and destination candidates. We propose Switching Head-Tail Funnel UNITER, which solves the task by predicting the target object and the destination individually using a single model. Our method is validated on a newly-built dataset consisting of object manipulation instructions and semi photo-realistic images captured in a standard Embodied AI simulator. The results show that our method outperforms the baseline method in terms of language comprehension accuracy. Furthermore, we conduct physical experiments in which a DSR delivers standardized everyday objects in a standardized domestic environment as requested by instructions with referring expressions. The experimental results show that the object grasping and placing actions are achieved with success rates of more than 90%.

==> tab/confusion_matrix_alfred-fc.tex <==
\begin{table}[t]
    \normalsize
    \caption{\small Confusion matrix on the ALFRED-fc dataset}
    \label{tab:confusion_matrix_alfred-fc}
    \centering
    \begin{tabular}{|c|c||cc|}
        \hline
        \multicolumn{2}{|c||}{} & \multicolumn{2}{c|}{Predicted Label} \\
        \cline{3-4}
        \multicolumn{2}{|c||}{} & \multicolumn{1}{c}{Positive} & \multicolumn{1}{c|}{Negative} \\
        \hline
        \hline
        True Label & Positive & 453 & 233 \\
        % \cline{2-4}
        & Negative & 24  & 662 \\
        \hline
    \end{tabular}
\end{table}
% TODO: 混同行列の書き方がこれで望ましいか
% スペースの都合で文にした


==> tab/params.tex <==
\begin{table}[t]
    \normalsize
    \centering
    \caption{\small Parameter settings of SHeFU}
    \label{tab:parameters}
    \begin{tabular}{|c|l|}
        \hline
        Optimizer & Adam\\ & ($\beta_1=0.9$, $\beta_2=0.999$)\\
        \hline
        Learning Rate & $8\times10^{-5}$\\
        \hline
        Step & $20000$\\
        \hline
        Batch Size & $8$\\
        \hline
        Dropout & $0.1$\\
        \hline
        Task Weights & $\lambda_\mathrm{targ}=1.0$, $\lambda_\mathrm{dest}=1.0$\\
        \hline
        \end{tabular}
\end{table}
% 余白の都合で文にする

